Conditional Variational Autoencoder with Balanced Pre-training for Generative Adversarial Networks

Class imbalance occurs in many real-world applications, including image classification, where the number of images in each class differs significantly. With imbalanced data, the generative adversarial networks (GANs) leans to majority class samples. The two recent methods, Balancing GAN (BAGAN) and improved BAGAN (BAGAN-GP), are proposed as an augmentation tool to handle this problem and restore the balance to the data. The former pre-trains the autoencoder weights in an unsupervised manner. However, it is unstable when the images from different categories have similar features. The latter is improved based on BAGAN by facilitating supervised autoencoder training, but the pre-training is biased towards the majority classes. In this work, we propose a novel Conditional Variational Autoencoder with Balanced Pre-training for Generative Adversarial Networks (CAPGAN) as an augmentation tool to generate realistic synthetic images. In particular, we utilize a conditional convolutional variational autoencoder with supervised and balanced pre-training for the GAN initialization and training with gradient penalty. Our proposed method presents a superior performance of other state-of-the-art methods on the highly imbalanced version of MNIST, Fashion-MNIST, CIFAR-10, and two medical imaging datasets. Our method can synthesize high-quality minority samples in terms of Fr\'echet inception distance, structural similarity index measure and perceptual quality.

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_breakhis.tex <==
\begin{table}
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{rlrrrr}
\toprule
                  &                 & \multicolumn{4}{c}{\textbf{BreakHis}}                                \\ \cmidrule{2-6} 
                  &                 & \multicolumn{2}{c}{Minority} & \multicolumn{2}{c}{Majority} \\
                  &                 & FID            & SSIM        & FID            & SSIM        \\
Imbalance Rate & Model & & & &             \\ \midrule

\multirow{3}{*}{2.19}
    & DCGAN & 456.39         & \num{5.66E-02}  & 294.23         & \num{6.34E-02}    
\\
& BAGAN-GP &  251.00         & \num{6.76E-02}        & 231.76         & \num{6.47E-02}        \\
& CAP-GAN & \textbf{237.47}         & \num{5.91E-02}        & \textbf{216.01}         & \num{6.06E-02}        \\ \cmidrule{2-6}

\multirow{3}{*}{10}
& DCGAN  & 565.67        &\num{5.25E-02}  & 416.73         & \num{5.86E-02}       \\
& BAGAN-GP & 211.28         & \num{8.95E-02}       &210.61         &\num{9.30E-02}       \\
& CAP-GAN & \textbf{203.60}        & \num{5.94E-02}        & \textbf{181.82}         & \num{5.95E-02}       \\

 \midrule
%  & & \multicolumn{2}{c}{FID} & \multicolumn{2}{c}{SSIM} \\
\multirow{2}{*}{Improvement on FID (\%) of 2.19} & CAP-GAN vs BAGAN-GP & \multicolumn{2}{c}{$5.39\uparrow$} &	\multicolumn{2}{c}{$6.79\uparrow$} \\
 & CAP-GAN vs DCGAN & \multicolumn{2}{c}{$47.97\uparrow$} &	\multicolumn{2}{c}{$26.58\uparrow$} \\ \cmidrule{2-6}
 
\multirow{2}{*}{Improvement on FID (\%) of 10} & CAP-GAN vs BAGAN-GP & \multicolumn{2}{c}{$3.63\uparrow$} &	\multicolumn{2}{c}{$13.67\uparrow$} \\
 & CAP-GAN vs DCGAN & \multicolumn{2}{c}{$64.01\uparrow$} &	\multicolumn{2}{c}{$56.37\uparrow$} \\
\bottomrule
\end{tabular}
}
\caption{FID and SSIM for BreakHis}
\label{tb_breakhis}
\end{table}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_cells.tex <==

\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rlrrrr}
\toprule
                  &                 & \multicolumn{4}{c}{\textbf{Cells}}                \\ \cmidrule{2-6} 
                  &                 & \multicolumn{2}{c}{avg(Minority)} & \multicolumn{2}{c}{Majority} \\
                  &                 & FID            & SSIM        & FID            & SSIM        \\
Imbalance Rate & Model &                &             &                &             \\ \midrule
\multirow{3}{*}{52.83} & DCGAN            & 438.48         &  \num{3.75E-01}       & 266.99         & \num{4.46E-01}        \\
 & BAGAN-GP            & 260.79        & \num{3.51E-01}        & 247.34         & \num{4.27E-01}        \\
 & CAP-GAN            & \textbf{228.76}         & \num{3.48E-01}        & \textbf{160.00}         & \num{4.35E-01}        \\ 
\midrule

\multirow{2}{*}{Improvement on FID (\%)} & CAP-GAN vs BAGAN-GP & \multicolumn{2}{c}{$12.28\uparrow$} & \multicolumn{2}{c}{$35.31\uparrow$} \\
 & CAP-GAN vs DCGAN & \multicolumn{2}{c}{$47.83\uparrow$} &	\multicolumn{2}{c}{$40.07\uparrow$} \\
\bottomrule
\end{tabular}
}
\caption{Averaged FID and SSIM for Cells}
\label{tb_cells}
\end{table}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_cells_det.tex <==
\begin{table}[!htbp]
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{rllrrrr}
\toprule

 & \multicolumn{1}{l}{} &  & \multicolumn{4}{c}{\textbf{Classes}} \\
\multicolumn{1}{l}{\begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular}} & Model &  & \textbf{0 (majority)} & \textbf{1} & \textbf{2} & \textbf{3} \\
 \midrule

\multirow{6}{*}{\textbf{52.83}} & \multirow{2}{*}{\textbf{DCGAN}} & \textbf{FID} & 266.99 & 431.15 & 460.66 & 423.63 \\
 &  & \textbf{SSIM} & \num{4.46E-01} & \num{3.08E-01} & \num{2.99E-01} & \num{5.19E-01} \\ \cmidrule{2-7} 
 
 & \multirow{2}{*}{\textbf{BAGAN-GP}} & \textbf{FID} & 272.94 & 284.52 & 339.98 & 291.15 \\
 &  & \textbf{SSIM} & \num{4.27E-01} & \num{2.84E-01} & \num{2.53E-01} & \num{5.19E-01} \\ \cmidrule{2-7} 
 
 & \multirow{2}{*}{\textbf{CAP-GAN}} & \textbf{FID} & \textbf{160.00} & \textbf{195.21} & \textbf{267.59} & \textbf{223.48} \\
 &  & \textbf{SSIM} & \num{4.35E-01} & \num{2.95E-01} & \num{2.58E-01} & \num{4.92E-01}\\

\bottomrule
\end{tabular}
}
\caption{FID and SSIM on Cells}
\label{tb_cells_det}
\end{table}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_cifar.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htbp]
\centering


\resizebox{\columnwidth}{!}{%
\begin{tabular}{rllrrrrrrrrrr}
\toprule
 &  &  & \multicolumn{10}{c}{\textbf{Classes}} \\
\begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular} & Model &  & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8 (majority)} & \textbf{9} \\
\midrule
%
%
\multirow{6}{*}{\textbf{5}} & \textbf{DCGAN} & \textbf{FID} & 335.43 & 482.27 & 449.98 & 455.06 & 435.90 & 498.40 & 401.05 & 1017.46 & 290.31 & 427.02 \\
 &  & \textbf{SSIM} & \num{9.30E-02} & \num{3.66E-02} & \num{6.68E-02} & \num{4.45E-02} & \num{6.34E-02} & \num{4.61E-02} & \num{5.44E-02} & \num{7.22E-02} & \num{7.78E-02} & \num{4.83E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 413.38 & 587.86 & 460.18 & 445.84 & 398.64 & 494.45 & 382.61 & 483.15 & 364.04 & 508.55 \\
 &  & \textbf{SSIM} & \num{8.74E-02} & \num{5.02E-02} & \num{7.01E-02} & \num{4.66E-02} & \num{6.69E-02} & \num{4.20E-02} & \num{5.51E-02} & \num{4.92E-02} & \num{8.94E-02} & \num{5.30E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{316.09} & \textbf{453.47} & \textbf{389.80} & \textbf{363.68} & \textbf{316.59} & \textbf{429.34} & \textbf{292.47} & \textbf{367.56} & \textbf{288.58} & \textbf{365.53} \\
 &  & \textbf{SSIM} & \num{8.67E-02} & \num{4.35E-02} & \num{7.34E-02} & \num{4.39E-02} & \num{6.80E-02} & \num{4.32E-02} & \num{5.46E-02} & \num{4.33E-02} & \num{8.14E-02} & \num{5.09E-02} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{10}} & \textbf{DCGAN} & \textbf{FID} & \textbf{335.43} & \textbf{482.27} & 449.98 & 455.06 & 435.90 & 498.40 & 401.05 & 1017.46 & \textbf{290.31} & 427.02 \\
 &  & \textbf{SSIM} & \num{9.30E-02} & \num{3.66E-02} & \num{6.68E-02} & \num{4.45E-02} & \num{6.34E-02} & \num{4.61E-02} & \num{5.44E-02} & \num{7.22E-02} & \num{7.78E-02} & \num{4.83E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 452.55 & 571.99 & 484.94 & 480.95 & 432.82 & 499.35 & 392.65 & 523.46 & 354.85 & 538.56 \\
 &  & \textbf{SSIM} & \num{8.37E-02} & \num{4.96E-02} & \num{7.06E-02} & \num{4.45E-02} & \num{6.72E-02} & \num{4.44E-02} & \num{5.44E-02} & \num{4.91E-02} & \num{9.06E-02} & \num{5.52E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & 343.25 & 484.30 & \textbf{402.93} & \textbf{403.45} & \textbf{347.28} & \textbf{464.23} & \textbf{333.19} & \textbf{411.61} & 291.54 & \textbf{402.40} \\
 &  & \textbf{SSIM} & \num{8.09E-02} & \num{4.51E-02} & \num{7.05E-02} & \num{4.48E-02} & \num{6.84E-02} & \num{4.27E-02} & \num{5.58E-02} & \num{4.66E-02} & \num{7.74E-02} & \num{5.25E-02} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{20}} & \textbf{DCGAN} & \textbf{FID} & 460.03 & 669.27 & 623.48 & 578.65 & 542.12 & 668.78 & 901.61 & 938.71 & 421.44 & 590.01 \\
 &  & \textbf{SSIM} & \num{8.69E-02} & \num{4.39E-02} & \num{6.30E-02} & \num{4.73E-02} & \num{6.56E-02} & \num{4.74E-02} & \num{5.16E-02} & \num{5.21E-02} & \num{8.06E-02} & \num{4.21E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 494.64 & 635.33 & 518.94 & 494.81 & 473.37 & 570.72 & 414.00 & 592.97 & 480.33 & 571.54 \\
 &  & \textbf{SSIM} & \num{7.18E-02} & \num{5.08E-02} & \num{6.66E-02} & \num{4.30E-02} & \num{6.38E-02} & \num{3.91E-02} & \num{5.68E-02} & \num{4.74E-02} & \num{7.40E-02} & \num{5.35E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{327.33} & \textbf{452.14} & \textbf{375.31} & \textbf{378.32} & \textbf{311.70} & \textbf{435.38} & \textbf{304.06} & \textbf{372.80} & \textbf{271.10} & \textbf{359.05} \\
 &  & \textbf{SSIM} & \num{8.53E-02} & \num{4.71E-02} & \num{7.44E-02} & \num{4.87E-02} & \num{6.87E-02} & \num{4.50E-02} & \num{5.35E-02} & \num{4.72E-02} & \num{8.29E-02} & \num{5.30E-02} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{50}} & \textbf{DCGAN} & \textbf{FID} & 453.33 & 704.75 & 714.18 & 791.47 & 589.46 & 837.46 & 970.32 & 805.21 & 518.52 & 751.53 \\
 &  & \textbf{SSIM} & \num{8.32E-02} & \num{5.15E-02} & \num{6.17E-02} & \num{4.42E-02} & \num{6.27E-02} & \num{4.47E-02} & \num{4.32E-02} & \num{4.82E-02} & \num{9.59E-02} & \num{6.20E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 468.87 & 580.71 & 537.93 & 525.67 & 474.88 & 573.96 & 400.66 & 608.49 & 455.16 & 569.07 \\
 &  & \textbf{SSIM} & \num{7.09E-02} & \num{5.36E-02} & \num{5.84E-02} & \num{4.05E-02} & \num{5.60E-02} & \num{3.97E-02} & \num{5.54E-02} & \num{4.11E-02} & \num{7.23E-02} & \num{4.94E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{334.77} & \textbf{478.42} & \textbf{375.97} & \textbf{435.97} & \textbf{369.53} & \textbf{501.21} & \textbf{334.56} & \textbf{414.94} & \textbf{346.43} & \textbf{455.75} \\
 &  & \textbf{SSIM} & \num{1.04E-01} & \num{5.44E-02} & \num{8.69E-02} & \num{5.59E-02} & \num{8.05E-02} & \num{5.50E-02} & \num{6.08E-02} & \num{5.15E-02} & \num{7.71E-02} & \num{6.15E-02} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{100}} & \textbf{DCGAN} & \textbf{FID} & 520.11 & 601.67 & 686.64 & 1171.73 & 614.79 & 719.38 & 536.56 & 858.94 & 525.37 & 598.75 \\
 &  & \textbf{SSIM} & \num{6.32E-02} & \num{5.35E-02} & \num{6.65E-02} & \num{4.17E-02} & \num{6.01E-02} & \num{3.25E-02} & \num{4.93E-02} & \num{4.35E-02} & \num{6.60E-02} & \num{5.98E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 494.84 & 578.75 & 556.39 & 582.14 & 510.50 & 630.90 & 477.23 & 634.04 & 456.06 & 527.54 \\
 &  & \textbf{SSIM} & \num{5.52E-02} & \num{4.84E-02} & \num{5.16E-02} & \num{3.76E-02} & \num{5.94E-02} & \num{3.55E-02} & \num{4.98E-02} & \num{4.00E-02} & \num{6.33E-02} & \num{4.76E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{303.45} & \textbf{383.25} & \textbf{366.81} & \textbf{436.42} & \textbf{338.91} & \textbf{483.67} & \textbf{299.45} & \textbf{356.86} & \textbf{339.45} & \textbf{368.58} \\
 &  & \textbf{SSIM} & \num{9.68E-02} & \num{5.69E-02} & \num{9.27E-02} & \num{5.86E-02} & \num{8.57E-02} & \num{5.47E-02} & \num{6.53E-02} & \num{5.35E-02} & \num{7.60E-02} & \num{6.34E-02} \\


\bottomrule
\end{tabular}%
}
\caption{Detailed FID and SSIM on CIFAR-10}
\label{tb_cifar}
\end{table}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_datasets.tex <==
\begin{table}[htb]
    \centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{|c||c|c||c|c|c|c|}
\hline & &  & \multicolumn{4}{c|} { Training Samples Per Class } \\
\cline { 4 - 7 } Dataset & Resolution & Class & Min & Median & Mean & Max \\
\hline \hline MNIST & $28 \times 28$ & 10 & 6000 & 6000 & 6,000 & 6000 \\
\hline Fashion-MNIST & $28 \times 28$ & 10 & 6000 & 6000 & 6000 & 6000 \\
\hline CIFAR-10 & $32 \times 32$ & 10 & 5,000 & 5,000 & 5,000 & 5,000 \\
\hline $BreakHis^{*}$ & $700 \times 460$ & 2 & 2,480 & N/A & N/A & 5,429 \\
\hline Cells & $100 \times 101$ & 4 & 106 & 887 & 1,721 & 5,600 \\
\hline
\end{tabular}}
    
    \caption{Datasets characterstics. BreakHis only has two classes so the median and mean are N/A's.}
    \label{tab:datasets}
\end{table}
%The numbers for BreakHis refer to the entire dataset.

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_fashion.tex <==

\begin{table}[!htbp]
\centering


\resizebox{\columnwidth}{!}{%
\begin{tabular}{rllrrrrrrrrrr}
\toprule
 &  &  & \multicolumn{10}{c}{\textbf{Classes}} \\
\begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular} & Model &  & \textbf{0 (majority)} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} \\
\midrule
%
%
\multirow{6}{*}{\textbf{5}} & \textbf{DCGAN} & \textbf{FID} & 316.61 & 335.28 & 270.11 & 321.86 & 243.71 & 467.57 & 304.32 & 517.13 & 359.43 & 600.26 \\
 &  & \textbf{SSIM} & \num{2.79E-01} & \num{4.67E-01} & \num{2.00E-01} & \num{2.61E-01} & \num{2.41E-01} & \num{1.53E-01} & \num{1.56E-01} & \num{3.44E-01} & \num{1.26E-01} & \num{3.94E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 240.21 & 198.58 & \textbf{219.04} & \textbf{227.59} & 217.74 & 312.32 & \textbf{199.81} & 422.22 & 266.23 & 339.90 \\
 &  & \textbf{SSIM} & \num{2.82E-01} & \num{5.07E-01} & \num{2.09E-01} & \num{2.89E-01} & \num{2.37E-01} & \num{1.54E-01} & \num{1.57E-01} & \num{3.68E-01} & \num{1.42E-01} & \num{3.36E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{232.47} & \textbf{188.72} & 227.35 & 266.68 & \textbf{213.06} & \textbf{294.53} & 253.16 & \textbf{371.26} & \textbf{255.98} & \textbf{311.13} \\
 &  & \textbf{SSIM} & \num{2.88E-01} & \num{5.05E-01} & \num{2.08E-01} & \num{2.85E-01} & \num{2.46E-01} & \num{1.52E-01} & \num{1.61E-01} & \num{3.70E-01} & \num{1.39E-01} & \num{3.36E-01} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{10}} & \textbf{DCGAN} & \textbf{FID} & 293.46 & 296.89 & 394.05 & 382.43 & 312.06 & 468.67 & 333.79 & 663.51 & 357.57 & 1,047.65 \\
 &  & \textbf{SSIM} & \num{2.96E-01} & \num{4.31E-01} & \num{2.10E-01} & \num{2.79E-01} & \num{2.43E-01} & \num{1.55E-01} & \num{1.54E-01} & \num{4.17E-01} & \num{1.31E-01} & \num{2.55E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 254.57 & 226.57 & 268.03 & 327.45 & 258.54 & 351.82 & 272.33 & 498.88 & 335.47 & 414.59 \\
 &  & \textbf{SSIM} & \num{3.03E-01} & \num{5.05E-01} & \num{2.10E-01} & \num{2.88E-01} & \num{2.35E-01} & \num{1.51E-01} & \num{1.61E-01} & \num{3.75E-01} & \num{1.50E-01} & \num{3.19E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{241.99} & \textbf{212.46} & \textbf{248.30} & \textbf{284.48} & \textbf{243.87} & \textbf{283.70} & \textbf{264.45} & \textbf{377.61} & \textbf{247.53} & \textbf{284.59} \\
 &  & \textbf{SSIM} & \num{2.94E-01} & \num{5.14E-01} & \num{2.21E-01} & \num{2.92E-01} & \num{2.55E-01} & \num{1.57E-01} & \num{1.74E-01} & \num{3.79E-01} & \num{1.49E-01} & \num{3.36E-01} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{20}} & \textbf{DCGAN} & \textbf{FID} & 468.58 & 354.95 & 495.27 & 517.65 & 459.10 & 418.44 & 844.35 & 588.78 & 418.41 & 491.40 \\
 &  & \textbf{SSIM} & \num{2.25E-01} & \num{5.33E-01} & \num{1.94E-01} & \num{3.07E-01} & \num{2.46E-01} & \num{1.48E-01} & \num{1.69E-01} & \num{3.53E-01} & \num{1.23E-01} & \num{3.35E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 288.96 & 203.21 & 276.49 & 293.31 & 275.66 & 378.25 & 290.71 & 477.10 & 359.08 & 376.68 \\
 &  & \textbf{SSIM} & \num{2.87E-01} & \num{5.01E-01} & \num{2.09E-01} & \num{2.90E-01} & \num{2.48E-01} & \num{1.57E-01} & \num{1.71E-01} & \num{3.63E-01} & \num{1.43E-01} & \num{3.37E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{230.71} & \textbf{194.39} & \textbf{228.56 }& \textbf{265.48} & \textbf{207.89} & \textbf{295.85} & \textbf{242.17} & \textbf{351.86} & \textbf{267.27} & \textbf{292.02} \\
 &  & \textbf{SSIM} & \num{2.98E-01} & \num{5.01E-01} & \num{2.24E-01} & \num{2.35E-01} & \num{2.48E-01} & \num{1.56E-01} & \num{1.72E-01} & \num{3.74E-01} & \num{1.40E-01} & \num{3.28E-01} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{50}} & \textbf{DCGAN} & \textbf{FID} & 514.94 & 422.51 & 453.95 & 427.50 & 492.23 & 456.38 & 889.33 & 631.19 & 519.58 & 568.42 \\
 &  & \textbf{SSIM} & \num{2.65E-01} & \num{5.57E-01} & \num{2.06E-01} & \num{2.88E-01} & \num{2.57E-01} & \num{1.72E-01} & \num{1.24E-01} & \num{3.80E-01} & \num{1.17E-01} & \num{3.60E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 317.47 & 355.79 & 330.91 & 329.52 & 300.14 & 393.50 & 320.05 & 564.54 & 392.19 & 510.76 \\
 &  & \textbf{SSIM} & \num{2.81E-01} & \num{5.02E-01} & \num{1.98E-01} & \num{2.72E-01} & \num{2.44E-01} & \num{1.38E-01} & \num{1.42E-01} & \num{3.35E-01} & \num{1.38E-01} & \num{3.19E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{225.08} & \textbf{212.64} & \textbf{225.52} & \textbf{281.69} & \textbf{206.58} & \textbf{294.37} & \textbf{241.84} & \textbf{378.05} & \textbf{262.33} & \textbf{311.76} \\
 &  & \textbf{SSIM} & \num{2.95E-01} & \num{5.10E-01} & \num{2.20E-01} & \num{2.87E-01} & \num{2.40E-01} & \num{1.56E-01} & \num{1.62E-01} & \num{3.80E-01} & \num{1.40E-01} & \num{3.39E-01} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{100}} & \textbf{DCGAN} & \textbf{FID} & 811.17 & 653.95 & 868.09 & 652.92 & 801.89 & 508.13 & 831.68 & 751.98 & 598.32 & 662.39 \\
 &  & \textbf{SSIM} & \num{2.69E-01} & \num{5.14E-01} & \num{2.21E-01} & \num{2.89E-01} & \num{2.74E-01} & \num{1.87E-01} & \num{1.91E-01} & \num{4.03E-01} & \num{1.01E-01} & \num{3.22E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 316.33 & 308.52 & 415.98 & 342.83 & 356.37 & 422.05 & 360.53 & 549.11 & 458.04 & 536.61 \\
 &  & \textbf{SSIM} & \num{2.70E-01} & \num{4.97E-01} & \num{2.11E-01} & \num{2.80E-01} & \num{2.33E-01} & \num{1.45E-01} & \num{1.56E-01} & \num{3.86E-01} & \num{1.47E-01} & \num{3.32E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{236.04} & \textbf{217.90} & \textbf{258.82} & \textbf{262.66} & \textbf{218.49} & \textbf{305.15} & \textbf{276.50} & \textbf{400.36} & \textbf{304.54} & \textbf{333.63} \\
 &  & \textbf{SSIM} & \num{2.94E-01} & \num{5.09E-01} & \num{2.04E-01} & \num{3.00E-01} & \num{2.38E-01} & \num{1.62E-01} & \num{1.59E-01} & \num{3.86E-01} & \num{1.41E-01} & \num{3.34E-01} \\

\bottomrule
\end{tabular}%
}
\caption{Detailed FID and SSIM on Fashion-MNIST}
\label{tb_fashion}
\end{table}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_milestone.tex <==
% \setlength{\tabcolsep}{18pt}
\begin{longtable}{|p{1.7cm}|p{7cm}|p{2cm}|p{2cm}|}
\caption{Project Milestones and Schedule}
\label{milestone}\\


\hline
\rowcolor[HTML]{FFCE93} 
\textbf{Milestone} & \textbf{Tasks} & \textbf{Reporting} & \textbf{End Date} \\ \hline
Week-1 & \begin{tabular}[c]{@{}l@{}}Literature Review: \\Traditional approaches for handling class\\imbalance (i.e. data-centric, model-centric\\and hybird method)
\end{tabular} &
\begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 15-08-2021 \\ \hline

Week-2 & \begin{tabular}[c]{@{}l@{}}Literature Review: \\Generative models and their applications\\for handling class imbalance\\ (i.e. GAN-based and VAE-based)\\Methodologies Exploration: \\Propose different frameworks and discuss\\within the team
\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 22-08-2021 \\ \hline

Week-3 & \begin{tabular}[c]{@{}l@{}}Literature Review: Medical imaging\\domain on class imbalance\\Research Domain Set Up
\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 29-08-2021 \\ \hline

Week-4 & \begin{tabular}[c]{@{}l@{}}GAN exploration on components and\\training strategies\\Datasets Exploration with statistical\\analysis
\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 05-09-2021 \\ \hline

\rowcolor[HTML]{FFCCC9} Week-5 & Proposal Report Finalization & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 12-09-2021 \\ \hline

Week-6 & \begin{tabular}[c]{@{}l@{}}BAGAN-GP experiments on MNIST, \\Fashion-MNIST and CIFAR10. Binary \\classification setting with imbalance \\rates of 1, 5, 10, 20, 50 and 100.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 19-09-2021 \\ \hline
Week-7 & \begin{tabular}[c]{@{}l@{}}BAGAN-GP experiments on Medical\\Imaging Data: Cells and BreakHis. \\Architecture exploration and adjustment \\based on BAGAN-GP\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 26-09-2021 \\ \hline
Week-8 & \begin{tabular}[c]{@{}l@{}}Develop our proposed model CAP-GAN: \\the CVAE component, new objective \\function and new GAN framework\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 10-10-2021 \\ \hline
\rowcolor[HTML]{FFCCC9} Week-9 & \begin{tabular}[c]{@{}l@{}} Complete the progress report. \\Implement pre-training for CVAE. \\BAGAN-GP experiments on MNIST, \\Fashion-MNIST and CIFAR10. 10-class \\classification setting with imbalance \\rates of 1, 5, 10, 20, 50 and 100.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 17-10-2021 \\ \hline

Week-10 & \begin{tabular}[c]{@{}l@{}}
Adjust the architecture of the proposed \\method. Conduct hyperparameter tuning \\for the proposed model. Evaluate the \\proposed model on all benchmark \\datasets. Re-evaluated BAGAN-GP for \\samples of different dimensions.
\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 24-10-2021 \\ \hline
Week-11 &\begin{tabular}[c]{@{}l@{}} Optimize the model performance in terms \\of the inference speed. Re-evaluate the \\optimized model. Summerize results and \\findings. Finalize the project title and \\model name. Draft the final report and \\finalize the documentations.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 31-10-2021 \\ \hline
 Week-12 &  \begin{tabular}[c]{@{}l@{}}
Develop the additional baseline model \\(i.e. conditional DCGAN). Evaluate \\the performance of the additional \\baseline model.
\\ Final report writing.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 07-11-2021 \\ \hline
\rowcolor[HTML]{FFCCC9} Week-13 &\begin{tabular}[c]{@{}l@{}} Finalize all results and documentations. \\Finalize the final report, presentation and \\artefacts. \end{tabular}& \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 14-11-2021 \\ \hline



\end{longtable}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_mnist.tex <==
% \begin{sidewaystable}[!htbp]
\begin{table}[!htbp]
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{rlcrrrrrrrrrr}
\toprule
 & \multicolumn{1}{l}{} &  & \multicolumn{10}{c}{\textbf{Classes}} \\
 \begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular} & Model &  & \textbf{0 (majority)} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} \\
\midrule
%
%
\multirow{6}{*}{\textbf{5}} & \textbf{DCGAN} & \textbf{FID} & 207.93 & 231.91 & 574.02 & 212.52 & 270.49 & 201.67 & 210.00 & 203.94 & 189.60 & 167.79 \\
 &  & \textbf{SSIM} & \num{2.96E-01} & \num{4.67E-01} & \num{1.75E-01} & \num{2.38E-01} & \num{2.28E-01} & \num{1.67E-01} & \num{2.29E-01} & \num{2.91E-01} & \num{2.30E-01} & \num{2.91E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 157.39 & \textbf{240.85} & 150.71 & 170.86 & 252.38 & 161.60 & 128.34 & 169.61 & 145.99 & 165.04 \\
 &  & \textbf{SSIM} & \num{2.86E-01} & \num{4.64E-01} & \num{1.71E-01} & \num{2.35E-01} & \num{2.20E-01} & \num{1.71E-01} & \num{2.36E-01} & \num{2.94E-01} & \num{2.16E-01} & \num{2.97E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{157.16} & 242.23 & \textbf{147.62} & \textbf{165.08} & \textbf{206.09 }& \textbf{154.53} & \textbf{127.52} & \textbf{145.89} & \textbf{145.70} & \textbf{155.65} \\
 &  & \textbf{SSIM} & \num{2.79E-01} & \num{4.74E-01} & \num{1.91E-01} & \num{2.49E-01} & \num{2.28E-01} & \num{1.80E-01} & \num{2.49E-01} & \num{3.09E-01} & \num{2.32E-01} & \num{3.08E-01} \\
\cmidrule{2-13}
%
%

\multirow{6}{*}{\textbf{10}} & \textbf{DCGAN} & \textbf{FID} & 528.09 & 242.10 & 180.30 & 206.94 & 250.58 & 230.72 & 201.96 & 228.18 & 187.70 & 192.01 \\
 &  & \textbf{SSIM} & \num{3.36E-01} & \num{4.58E-01} & \num{1.87E-01} & \num{2.27E-01} & \num{2.38E-01} & \num{1.70E-01} & \num{2.49E-01} & \num{2.68E-01} & \num{2.27E-01} & \num{2.97E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 165.08 & 282.54 & 155.78 & 178.82 & 237.48 & 177.91 & \textbf{138.46} & 198.25 & 159.68 & 158.06 \\
 &  & \textbf{SSIM} &  \num{2.70E-01} & \num{4.66E-01} & \num{1.74E-01} & \num{2.34E-01} & \num{2.32E-01} & \num{1.72E-01} & \num{2.44E-01} & \num{3.10E-01} & \num{2.29E-01} & \num{2.98E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{160.12} & \textbf{250.68} & \textbf{145.18} & \textbf{174.58} & \textbf{225.67} & \textbf{177.76} & 146.50 & \textbf{163.00} & \textbf{157.12} & \textbf{154.49} \\
 &  & \textbf{SSIM} & \num{2.90E-01} & \num{4.78E-01} & \num{1.79E-01} & \num{2.40E-01} & \num{2.28E-01} & \num{1.72E-01} & \num{2.48E-01} & \num{2.98E-01} & \num{2.30E-01} & \num{3.01E-01} \\
\cmidrule{2-13}
%
%

\multirow{6}{*}{\textbf{20}} & \textbf{DCGAN} & \textbf{FID} & 210.22 & 344.15 & 508.33 & 184.82 & 317.27 & 205.03 & 184.93 & 301.06 & 239.51 & 224.13 \\
 &  & \textbf{SSIM} & \num{2.85E-01} & \num{4.69E-01} & \num{2.06E-01} & \num{2.06E-01} & \num{2.31E-01} & \num{1.65E-01} & \num{2.70E-01} & \num{3.23E-01} & \num{2.43E-01} & \num{3.02E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 174.21 & 257.86 & 178.63 & 180.72 & 244.97 & \textbf{186.60} & 138.85 & 210.84 & 171.13 & 171.02 \\
 &  & \textbf{SSIM} &  \num{2.78E-01} & \num{4.68E-01} & \num{1.75E-01} & \num{2.28E-01} & \num{2.40E-01} & \num{1.74E-01} & \num{2.49E-01} & \num{3.19E-01} & \num{2.24E-01} & \num{3.22E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{149.04} & \textbf{219.41} & \textbf{161.04} & \textbf{155.32} & \textbf{243.29} & 188.62 & \textbf{136.91} & \textbf{147.25} & \textbf{156.50} & \textbf{154.00} \\
 &  & \textbf{SSIM} & \num{2.86E-01} & \num{4.63E-01} & \num{1.88E-01} & \num{2.47E-01} & \num{2.31E-01} & \num{1.87E-01} & \num{2.59E-01} & \num{3.03E-01} & \num{2.38E-01} & \num{3.12E-01} \\
\cmidrule{2-13}
%
%

\multirow{6}{*}{\textbf{50}} & \textbf{DCGAN} & \textbf{FID} & 722.07 & 528.49 & 619.79 & 350.49 & 483.00 & 435.90 & 558.23 & 419.34 & 519.03 & 402.41 \\
 &  & \textbf{SSIM} & \num{3.13E-01} & \num{3.58E-01} & \num{1.68E-01} & \num{2.13E-01} & \num{2.43E-01} & \num{2.32E-01} & \num{2.36E-01} & \num{3.10E-01} & \num{2.08E-01} & \num{3.26E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & \textbf{149.28} & 250.79 & 197.96 & 180.09 & 277.71 & 200.27 & 163.66 & 176.13 & 194.40 & 201.32 \\
 &  & \textbf{SSIM} &  \num{2.79E-01} & \num{4.58E-01} & \num{1.77E-01} & \num{2.30E-01} & \num{2.23E-01} & \num{1.66E-01} & \num{2.47E-01} & \num{2.99E-01} & \num{2.27E-01} & \num{2.91E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & 163.90 & \textbf{233.15} & \textbf{157.93} & \textbf{156.78} & \textbf{242.64} & \textbf{173.47} & \textbf{145.42} & \textbf{160.22} & \textbf{148.28} & \textbf{170.29} \\
 &  & \textbf{SSIM} & \num{2.83E-01} & \num{4.69E-01} & \num{1.72E-01} & \num{2.33E-01} & \num{2.14E-01} & \num{1.66E-01} & \num{2.50E-01} & \num{2.90E-01} & \num{2.30E-01} & \num{3.04E-01} \\
\cmidrule{2-13}
%
%

\multirow{6}{*}{\textbf{100}} & \textbf{DCGAN} & \textbf{FID} & 711.49 & 505.38 & 418.74 & 565.95 & 449.87 & 605.25 & 456.66 & 494.41 & 544.54 & 561.03 \\
 &  & \textbf{SSIM} & \num{1.68E-01} & \num{1.50E-01} & \num{1.13E-01} & \num{1.40E-01} & \num{2.78E-01} & \num{8.79E-02} & \num{2.43E-01} & \num{1.83E-01} & \num{1.63E-01} & \num{2.91E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 167.74 & 237.99 & 215.68 & 203.27 & 280.70 & 230.98 & 228.46 & 228.21 & 221.93 & 206.48 \\
 &  & \textbf{SSIM} &  \num{2.79E-01} & \num{4.62E-01} & \num{1.77E-01} & \num{2.09E-01} & \num{2.30E-01} & \num{1.55E-01} & \num{2.47E-01} & \num{2.85E-01} & \num{2.27E-01} & \num{2.92E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{160.88} & \textbf{210.50} & \textbf{154.40} & \textbf{155.25} & \textbf{202.50} & \textbf{173.52} & \textbf{139.23} & \textbf{166.63} & \textbf{153.39} & \textbf{156.62 }\\
 &  & \textbf{SSIM} & \num{2.81E-01} & \num{4.83E-01} & \num{1.69E-01} & \num{2.33E-01} & \num{2.35E-01} & \num{1.70E-01} & \num{2.71E-01} & \num{2.91E-01} & \num{2.25E-01} & \num{3.12E-01} \\
%
%

\bottomrule
\end{tabular}%
}
\caption{Detailed FID and SSIM on MNIST}
\label{tb_mnist}
\end{table}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_param.tex <==
\begin{table}[h]
\centering

\resizebox{\linewidth}{!}{%
\begin{tabular}{lc}
\hlineB{3}
           Hyperparameter                    & Values                                                                \\ \cline{1-2} 



Learning Rate (CVAE)          & 0.0006, 0.0007, 0.0008, 0.001, 0.0005                                 \\
CVAE Epoch                    & 30, 40, 50                                                            \\
Adam beta1 (CVAE)                & 0.5, 0.6, 0.7, 0.8                                                    \\ 
Learning Rate (Generator)     & 0.00005, 0.0001, 0.0002, 0.0005, 0.0008, 0.0013, 0.0015, 0.001, 0.002 \\
Learning Rate (Discriminator) & 0.00005, 0.0001, 0.0008, 0.0013, 0.0015, 0.0002, 0.002                \\
Gradient Penalty Weight                     & 5, 10                                                                 \\
Train Ratio                     & 2, 3, 4, 5, 6, 7, 8, 10                                               \\

Batch Size                    & 32, 64, 128, 256                                                      \\
Latent Dimension                    & 64, 128, 256, 512                                                     \\

\hlineB{3}
\end{tabular}%
}
\caption{Hyperparameter Optimization for CAP-GAN}
\label{tab:hyperparameter}
\end{table}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_summary.tex <==
\begin{table*}[t]
\centering

\resizebox{\linewidth}{!}{%
\begin{tabular}{rlrrrrrrrrrrrr}
\toprule
                                                                              &                                                           & \multicolumn{4}{c}{\textbf{MNIST}}                               & \multicolumn{4}{c}{\textbf{Fashion-MNIST}}                       & \multicolumn{4}{c}{\textbf{CIFAR-10}}                             \\ \cmidrule{2-14} 
                                                                              &                                                           & \multicolumn{2}{c}{avg(Minority)} & \multicolumn{2}{c}{Majority} & \multicolumn{2}{c}{avg(Minority)} & \multicolumn{2}{c}{Majority} & \multicolumn{2}{c}{avg(Minority)} & \multicolumn{2}{c}{Majority} \\
 &  & FID & SSIM & FID & SSIM & FID & SSIM & FID & SSIM & FID & SSIM & FID & SSIM \\
\begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular} & Model &  &  &  &  &  &  &  &  &  &  &  &  \\ \midrule

\multirow{3}{*}{5} & DCGAN & 251.33 & \num{2.57E-01} & 207.93 & $\mathbf{2.96\times10^{-1}}$ & 379.96 & \num{2.60E-01} & 316.61 & \num{2.79E-01} & 495.27 & \num{5.67E-02} & 335.43 & $\mathbf{9.30\times10^{-2}}$ \\
 & BAGAN-GP & 176.15 & \num{2.56E-01} & 157.39 & \num{2.86E-01} & 267.05 & $\mathbf{2.67\times10^{-1}}$ & 240.21 & \num{2.82E-01} & 463.85 & \num{5.78E-02} & 364.04 & \num{8.94E-02} \\
 & CAP-GAN & \textbf{165.59} & $\mathbf{2.69\times10^{-1}}$ & \textbf{157.16} & \num{2.79E-01} & \textbf{264.65} & $\mathbf{2.67\times10^{-1}}$ & \textbf{232.47} & $\mathbf{2.88\times10^{-1}}$ & \textbf{366.06} & $\mathbf{6.00\times10^{-2}}$ & \textbf{288.58} & \num{8.00E-02} \\ \cmidrule{2-14} 
 
\multirow{3}{*}{10} & DCGAN & 213.39 & \num{2.58E-01} & 528.09 & \num{3.36E-01} & 472.96 & \num{2.53E-01} & 293.46 & \num{2.96E-01} & 495.27 & \num{5.67E-02} & 335.43 & $\mathbf{9.30\times10^{-2}}$ \\
 & BAGAN-GP & 187.44 & \num{2.62E-01} & 165.08 & \num{2.70E-01} & 328.19 & \num{2.66E-01} & 254.57 & $\mathbf{3.03\times10^{-1}}$ & 486.36 & \num{5.76E-02} & 354.85 & \num{9.06E-02} \\
 & CAP-GAN & \textbf{177.22} & $\mathbf{2.64\times10^{-1}}$ & \textbf{160.12} & $\mathbf{2.90\times10^{-1}}$ & \textbf{271.89} & $\mathbf{2.75\times10^{-1}}$ & \textbf{241.99} & \num{2.94E-01} & \textbf{399.1}8 & $\mathbf{6.00\times10^{-2}}$ & \textbf{291.54} & \num{8.00E-02} \\ \cmidrule{2-14}


\multirow{3}{*}{20} & DCGAN & 278.80 & \num{2.68E-01} & 210.22 & \num{2.85E-01} & 509.82 & \num{2.67E-01} & 468.58 & \num{2.25E-01} & 659.34 & \num{5.48E-02} & 460.03 & $\mathbf{8.69\times10^{-2}}$ \\
 & BAGAN-GP & 193.40 & \num{2.66E-01} & 174.21 & \num{2.78E-01} & 325.61 & $\mathbf{2.69\times10^{-1}}$ & 288.96 & \num{2.87E-01} & 529.59 & \num{5.48E-02} & 480.33 & \num{7.40E-02} \\
 & CAP-GAN & \textbf{173.59} & $\mathbf{2.70\times10^{-1}}$ & \textbf{149.04} & $\mathbf{2.86\times10^{-1}}$ & \textbf{260.61} & \num{2.64E-01} & \textbf{230.71} & $\mathbf{2.98\times10^{-1}}$ & \textbf{368.46} & $\mathbf{6.00\times10^{-2}}$ & \textbf{271.10} & \num{8.00E-02} \\ \cmidrule{2-14}
 

\multirow{3}{*}{50} & DCGAN & 479.63 & \num{2.55E-01} & 722.07 & \num{3.13E-01} & 540.12 & $\mathbf{2.74\times10^{-1}}$ & 514.94 & \num{2.65E-01} & 742.54 & \num{5.71E-02} & 453.33 & $\mathbf{8.32\times10^{-2}}$ \\
 & BAGAN-GP & 204.70 & \num{2.58E-01} & \textbf{149.28} & \num{2.79E-01} & 388.60 & \num{2.54E-01} & 317.47 & \num{2.81E-01} & 529.69 & \num{5.17E-02} & 455.16 & \num{7.23E-02} \\
 & CAP-GAN & \textbf{176.47} & $\mathbf{2.59\times10^{-1}}$ & 163.90 & $\mathbf{2.83\times10^{-1}}$ & \textbf{268.31} & \num{2.70E-01} & \textbf{225.08} & $\mathbf{2.95\times10^{-1}}$ & \textbf{411.23} & $\mathbf{7.00\times10^{-2}}$ & \textbf{346.43} & \num{8.00E-02} \\ \cmidrule{2-14}
 

\multirow{3}{*}{100} & DCGAN & 511.31 & \num{1.83E-01} & 711.49 & \num{1.68E-01} & 703.26 & $\mathbf{2.78\times10^{-1}}$ & 811.17 & \num{2.69E-01} & 701.54 & \num{5.26E-02} & 520.11 & \num{6.32E-02} \\ 
 & BAGAN-GP & 228.19 & \num{2.54E-01} & 167.74 & \num{2.79E-01} & 416.67 & \num{2.65E-01} & 316.33 & \num{2.70E-01} & 554.70 & \num{4.72E-02} & 456.06 & \num{6.33E-02} \\
 & CAP-GAN & \textbf{168.00} & $\mathbf{2.66\times10^{-1}}$ & \textbf{160.88} & $\mathbf{2.81\times10^{-1}}$ & \textbf{286.45} & \num{2.70E-01} & \textbf{236.04} & $\mathbf{2.94\times10^{-1}}$ & \textbf{370.82} & $\mathbf{7.00\times10^{-2}}$ & \textbf{339.45} & $\mathbf{8.00\times10^{-2}}$ \\ 


\midrule
\multirow{3}{*}{p-value} & & \multicolumn{2}{c}{FID} & \multicolumn{2}{c}{SSIM} & \multicolumn{2}{c}{FID} & \multicolumn{2}{c}{SSIM} & \multicolumn{2}{c}{FID} & \multicolumn{2}{c}{SSIM} \\

 & CAP-GAN vs BAGAN-GP & \multicolumn{2}{c}{\num{1.3E-03}} & \multicolumn{2}{c}{\num{7.1E-01}} & \multicolumn{2}{c}{\num{5.0E-06}} & \multicolumn{2}{c}{\num{8.0E-01}} & \multicolumn{2}{c}{\num{5.0E-16}} & \multicolumn{2}{c}{\num{3.3E-02}} \\

 & CAP-GAN vs DCGAN & \multicolumn{2}{c}{\num{2.8E-12}} & \multicolumn{2}{c}{\num{2.4E-01}} & \multicolumn{2}{c}{\num{8.9E-15}} & \multicolumn{2}{c}{\num{8.1E-01}} & \multicolumn{2}{c}{\num{4.5E-11}} & \multicolumn{2}{c}{\num{1.5E-01}} \\

\bottomrule
\end{tabular}%
}
\caption{Averaged FID and SSIM for General Vision Benchmarks}
\label{tb_summary}
\end{table*}

==> IJCAI--22 CAP-GAN_arxiv/tables/tb_time.tex <==

\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrr}
\toprule
Dataset      & Each CVAE Epoch (s)  & Each GAN Epoch (s) \\ \cmidrule{1-3} 
MNIST         & 3.34 & 55.45                  \\
Fashion-MNIST & 3.43 & 55.80                  \\
CIFAR10       & 3.94 & 90.44                 \\
Cells         & 2.06 & 41.13            \\
BreakHis      & 0.79 & 32.70                \\ 
\bottomrule
\end{tabular}%
}
\caption{Estimation of Computational Time for Different Datasets}
\label{tb_time}
\end{table}

==> tables/tb_cells_det.tex <==
\begin{table}[!htbp]
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{rllrrrr}
\toprule

 & \multicolumn{1}{l}{} &  & \multicolumn{4}{c}{\textbf{Classes}} \\
\multicolumn{1}{l}{\begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular}} & Model &  & \textbf{0 (majority)} & \textbf{1} & \textbf{2} & \textbf{3} \\
 \midrule

\multirow{6}{*}{\textbf{52.83}} & \multirow{2}{*}{\textbf{DCGAN}} & \textbf{FID} & 266.99 & 431.15 & 460.66 & 423.63 \\
 &  & \textbf{SSIM} & \num{4.46E-01} & \num{3.08E-01} & \num{2.99E-01} & \num{5.19E-01} \\ \cmidrule{2-7} 
 
 & \multirow{2}{*}{\textbf{BAGAN-GP}} & \textbf{FID} & 272.94 & 284.52 & 339.98 & 291.15 \\
 &  & \textbf{SSIM} & \num{4.27E-01} & \num{2.84E-01} & \num{2.53E-01} & \num{5.19E-01} \\ \cmidrule{2-7} 
 
 & \multirow{2}{*}{\textbf{CAP-GAN}} & \textbf{FID} & \textbf{160.00} & \textbf{195.21} & \textbf{267.59} & \textbf{223.48} \\
 &  & \textbf{SSIM} & \num{4.35E-01} & \num{2.95E-01} & \num{2.58E-01} & \num{4.92E-01}\\

\bottomrule
\end{tabular}
}
\caption{FID and SSIM on Cells}
\label{tb_cells_det}
\end{table}

==> tables/tb_cifar.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htbp]
\centering


\resizebox{\columnwidth}{!}{%
\begin{tabular}{rllrrrrrrrrrr}
\toprule
 &  &  & \multicolumn{10}{c}{\textbf{Classes}} \\
\begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular} & Model &  & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8 (majority)} & \textbf{9} \\
\midrule
%
%
\multirow{6}{*}{\textbf{5}} & \textbf{DCGAN} & \textbf{FID} & 335.43 & 482.27 & 449.98 & 455.06 & 435.90 & 498.40 & 401.05 & 1017.46 & 290.31 & 427.02 \\
 &  & \textbf{SSIM} & \num{9.30E-02} & \num{3.66E-02} & \num{6.68E-02} & \num{4.45E-02} & \num{6.34E-02} & \num{4.61E-02} & \num{5.44E-02} & \num{7.22E-02} & \num{7.78E-02} & \num{4.83E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 413.38 & 587.86 & 460.18 & 445.84 & 398.64 & 494.45 & 382.61 & 483.15 & 364.04 & 508.55 \\
 &  & \textbf{SSIM} & \num{8.74E-02} & \num{5.02E-02} & \num{7.01E-02} & \num{4.66E-02} & \num{6.69E-02} & \num{4.20E-02} & \num{5.51E-02} & \num{4.92E-02} & \num{8.94E-02} & \num{5.30E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{316.09} & \textbf{453.47} & \textbf{389.80} & \textbf{363.68} & \textbf{316.59} & \textbf{429.34} & \textbf{292.47} & \textbf{367.56} & \textbf{288.58} & \textbf{365.53} \\
 &  & \textbf{SSIM} & \num{8.67E-02} & \num{4.35E-02} & \num{7.34E-02} & \num{4.39E-02} & \num{6.80E-02} & \num{4.32E-02} & \num{5.46E-02} & \num{4.33E-02} & \num{8.14E-02} & \num{5.09E-02} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{10}} & \textbf{DCGAN} & \textbf{FID} & \textbf{335.43} & \textbf{482.27} & 449.98 & 455.06 & 435.90 & 498.40 & 401.05 & 1017.46 & \textbf{290.31} & 427.02 \\
 &  & \textbf{SSIM} & \num{9.30E-02} & \num{3.66E-02} & \num{6.68E-02} & \num{4.45E-02} & \num{6.34E-02} & \num{4.61E-02} & \num{5.44E-02} & \num{7.22E-02} & \num{7.78E-02} & \num{4.83E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 452.55 & 571.99 & 484.94 & 480.95 & 432.82 & 499.35 & 392.65 & 523.46 & 354.85 & 538.56 \\
 &  & \textbf{SSIM} & \num{8.37E-02} & \num{4.96E-02} & \num{7.06E-02} & \num{4.45E-02} & \num{6.72E-02} & \num{4.44E-02} & \num{5.44E-02} & \num{4.91E-02} & \num{9.06E-02} & \num{5.52E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & 343.25 & 484.30 & \textbf{402.93} & \textbf{403.45} & \textbf{347.28} & \textbf{464.23} & \textbf{333.19} & \textbf{411.61} & 291.54 & \textbf{402.40} \\
 &  & \textbf{SSIM} & \num{8.09E-02} & \num{4.51E-02} & \num{7.05E-02} & \num{4.48E-02} & \num{6.84E-02} & \num{4.27E-02} & \num{5.58E-02} & \num{4.66E-02} & \num{7.74E-02} & \num{5.25E-02} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{20}} & \textbf{DCGAN} & \textbf{FID} & 460.03 & 669.27 & 623.48 & 578.65 & 542.12 & 668.78 & 901.61 & 938.71 & 421.44 & 590.01 \\
 &  & \textbf{SSIM} & \num{8.69E-02} & \num{4.39E-02} & \num{6.30E-02} & \num{4.73E-02} & \num{6.56E-02} & \num{4.74E-02} & \num{5.16E-02} & \num{5.21E-02} & \num{8.06E-02} & \num{4.21E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 494.64 & 635.33 & 518.94 & 494.81 & 473.37 & 570.72 & 414.00 & 592.97 & 480.33 & 571.54 \\
 &  & \textbf{SSIM} & \num{7.18E-02} & \num{5.08E-02} & \num{6.66E-02} & \num{4.30E-02} & \num{6.38E-02} & \num{3.91E-02} & \num{5.68E-02} & \num{4.74E-02} & \num{7.40E-02} & \num{5.35E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{327.33} & \textbf{452.14} & \textbf{375.31} & \textbf{378.32} & \textbf{311.70} & \textbf{435.38} & \textbf{304.06} & \textbf{372.80} & \textbf{271.10} & \textbf{359.05} \\
 &  & \textbf{SSIM} & \num{8.53E-02} & \num{4.71E-02} & \num{7.44E-02} & \num{4.87E-02} & \num{6.87E-02} & \num{4.50E-02} & \num{5.35E-02} & \num{4.72E-02} & \num{8.29E-02} & \num{5.30E-02} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{50}} & \textbf{DCGAN} & \textbf{FID} & 453.33 & 704.75 & 714.18 & 791.47 & 589.46 & 837.46 & 970.32 & 805.21 & 518.52 & 751.53 \\
 &  & \textbf{SSIM} & \num{8.32E-02} & \num{5.15E-02} & \num{6.17E-02} & \num{4.42E-02} & \num{6.27E-02} & \num{4.47E-02} & \num{4.32E-02} & \num{4.82E-02} & \num{9.59E-02} & \num{6.20E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 468.87 & 580.71 & 537.93 & 525.67 & 474.88 & 573.96 & 400.66 & 608.49 & 455.16 & 569.07 \\
 &  & \textbf{SSIM} & \num{7.09E-02} & \num{5.36E-02} & \num{5.84E-02} & \num{4.05E-02} & \num{5.60E-02} & \num{3.97E-02} & \num{5.54E-02} & \num{4.11E-02} & \num{7.23E-02} & \num{4.94E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{334.77} & \textbf{478.42} & \textbf{375.97} & \textbf{435.97} & \textbf{369.53} & \textbf{501.21} & \textbf{334.56} & \textbf{414.94} & \textbf{346.43} & \textbf{455.75} \\
 &  & \textbf{SSIM} & \num{1.04E-01} & \num{5.44E-02} & \num{8.69E-02} & \num{5.59E-02} & \num{8.05E-02} & \num{5.50E-02} & \num{6.08E-02} & \num{5.15E-02} & \num{7.71E-02} & \num{6.15E-02} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{100}} & \textbf{DCGAN} & \textbf{FID} & 520.11 & 601.67 & 686.64 & 1171.73 & 614.79 & 719.38 & 536.56 & 858.94 & 525.37 & 598.75 \\
 &  & \textbf{SSIM} & \num{6.32E-02} & \num{5.35E-02} & \num{6.65E-02} & \num{4.17E-02} & \num{6.01E-02} & \num{3.25E-02} & \num{4.93E-02} & \num{4.35E-02} & \num{6.60E-02} & \num{5.98E-02} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 494.84 & 578.75 & 556.39 & 582.14 & 510.50 & 630.90 & 477.23 & 634.04 & 456.06 & 527.54 \\
 &  & \textbf{SSIM} & \num{5.52E-02} & \num{4.84E-02} & \num{5.16E-02} & \num{3.76E-02} & \num{5.94E-02} & \num{3.55E-02} & \num{4.98E-02} & \num{4.00E-02} & \num{6.33E-02} & \num{4.76E-02} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{303.45} & \textbf{383.25} & \textbf{366.81} & \textbf{436.42} & \textbf{338.91} & \textbf{483.67} & \textbf{299.45} & \textbf{356.86} & \textbf{339.45} & \textbf{368.58} \\
 &  & \textbf{SSIM} & \num{9.68E-02} & \num{5.69E-02} & \num{9.27E-02} & \num{5.86E-02} & \num{8.57E-02} & \num{5.47E-02} & \num{6.53E-02} & \num{5.35E-02} & \num{7.60E-02} & \num{6.34E-02} \\


\bottomrule
\end{tabular}%
}
\caption{Detailed FID and SSIM on CIFAR-10}
\label{tb_cifar}
\end{table}

==> tables/tb_fashion.tex <==

\begin{table}[!htbp]
\centering


\resizebox{\columnwidth}{!}{%
\begin{tabular}{rllrrrrrrrrrr}
\toprule
 &  &  & \multicolumn{10}{c}{\textbf{Classes}} \\
\begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular} & Model &  & \textbf{0 (majority)} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} \\
\midrule
%
%
\multirow{6}{*}{\textbf{5}} & \textbf{DCGAN} & \textbf{FID} & 316.61 & 335.28 & 270.11 & 321.86 & 243.71 & 467.57 & 304.32 & 517.13 & 359.43 & 600.26 \\
 &  & \textbf{SSIM} & \num{2.79E-01} & \num{4.67E-01} & \num{2.00E-01} & \num{2.61E-01} & \num{2.41E-01} & \num{1.53E-01} & \num{1.56E-01} & \num{3.44E-01} & \num{1.26E-01} & \num{3.94E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 240.21 & 198.58 & \textbf{219.04} & \textbf{227.59} & 217.74 & 312.32 & \textbf{199.81} & 422.22 & 266.23 & 339.90 \\
 &  & \textbf{SSIM} & \num{2.82E-01} & \num{5.07E-01} & \num{2.09E-01} & \num{2.89E-01} & \num{2.37E-01} & \num{1.54E-01} & \num{1.57E-01} & \num{3.68E-01} & \num{1.42E-01} & \num{3.36E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{232.47} & \textbf{188.72} & 227.35 & 266.68 & \textbf{213.06} & \textbf{294.53} & 253.16 & \textbf{371.26} & \textbf{255.98} & \textbf{311.13} \\
 &  & \textbf{SSIM} & \num{2.88E-01} & \num{5.05E-01} & \num{2.08E-01} & \num{2.85E-01} & \num{2.46E-01} & \num{1.52E-01} & \num{1.61E-01} & \num{3.70E-01} & \num{1.39E-01} & \num{3.36E-01} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{10}} & \textbf{DCGAN} & \textbf{FID} & 293.46 & 296.89 & 394.05 & 382.43 & 312.06 & 468.67 & 333.79 & 663.51 & 357.57 & 1,047.65 \\
 &  & \textbf{SSIM} & \num{2.96E-01} & \num{4.31E-01} & \num{2.10E-01} & \num{2.79E-01} & \num{2.43E-01} & \num{1.55E-01} & \num{1.54E-01} & \num{4.17E-01} & \num{1.31E-01} & \num{2.55E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 254.57 & 226.57 & 268.03 & 327.45 & 258.54 & 351.82 & 272.33 & 498.88 & 335.47 & 414.59 \\
 &  & \textbf{SSIM} & \num{3.03E-01} & \num{5.05E-01} & \num{2.10E-01} & \num{2.88E-01} & \num{2.35E-01} & \num{1.51E-01} & \num{1.61E-01} & \num{3.75E-01} & \num{1.50E-01} & \num{3.19E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{241.99} & \textbf{212.46} & \textbf{248.30} & \textbf{284.48} & \textbf{243.87} & \textbf{283.70} & \textbf{264.45} & \textbf{377.61} & \textbf{247.53} & \textbf{284.59} \\
 &  & \textbf{SSIM} & \num{2.94E-01} & \num{5.14E-01} & \num{2.21E-01} & \num{2.92E-01} & \num{2.55E-01} & \num{1.57E-01} & \num{1.74E-01} & \num{3.79E-01} & \num{1.49E-01} & \num{3.36E-01} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{20}} & \textbf{DCGAN} & \textbf{FID} & 468.58 & 354.95 & 495.27 & 517.65 & 459.10 & 418.44 & 844.35 & 588.78 & 418.41 & 491.40 \\
 &  & \textbf{SSIM} & \num{2.25E-01} & \num{5.33E-01} & \num{1.94E-01} & \num{3.07E-01} & \num{2.46E-01} & \num{1.48E-01} & \num{1.69E-01} & \num{3.53E-01} & \num{1.23E-01} & \num{3.35E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 288.96 & 203.21 & 276.49 & 293.31 & 275.66 & 378.25 & 290.71 & 477.10 & 359.08 & 376.68 \\
 &  & \textbf{SSIM} & \num{2.87E-01} & \num{5.01E-01} & \num{2.09E-01} & \num{2.90E-01} & \num{2.48E-01} & \num{1.57E-01} & \num{1.71E-01} & \num{3.63E-01} & \num{1.43E-01} & \num{3.37E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{230.71} & \textbf{194.39} & \textbf{228.56 }& \textbf{265.48} & \textbf{207.89} & \textbf{295.85} & \textbf{242.17} & \textbf{351.86} & \textbf{267.27} & \textbf{292.02} \\
 &  & \textbf{SSIM} & \num{2.98E-01} & \num{5.01E-01} & \num{2.24E-01} & \num{2.35E-01} & \num{2.48E-01} & \num{1.56E-01} & \num{1.72E-01} & \num{3.74E-01} & \num{1.40E-01} & \num{3.28E-01} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{50}} & \textbf{DCGAN} & \textbf{FID} & 514.94 & 422.51 & 453.95 & 427.50 & 492.23 & 456.38 & 889.33 & 631.19 & 519.58 & 568.42 \\
 &  & \textbf{SSIM} & \num{2.65E-01} & \num{5.57E-01} & \num{2.06E-01} & \num{2.88E-01} & \num{2.57E-01} & \num{1.72E-01} & \num{1.24E-01} & \num{3.80E-01} & \num{1.17E-01} & \num{3.60E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 317.47 & 355.79 & 330.91 & 329.52 & 300.14 & 393.50 & 320.05 & 564.54 & 392.19 & 510.76 \\
 &  & \textbf{SSIM} & \num{2.81E-01} & \num{5.02E-01} & \num{1.98E-01} & \num{2.72E-01} & \num{2.44E-01} & \num{1.38E-01} & \num{1.42E-01} & \num{3.35E-01} & \num{1.38E-01} & \num{3.19E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{225.08} & \textbf{212.64} & \textbf{225.52} & \textbf{281.69} & \textbf{206.58} & \textbf{294.37} & \textbf{241.84} & \textbf{378.05} & \textbf{262.33} & \textbf{311.76} \\
 &  & \textbf{SSIM} & \num{2.95E-01} & \num{5.10E-01} & \num{2.20E-01} & \num{2.87E-01} & \num{2.40E-01} & \num{1.56E-01} & \num{1.62E-01} & \num{3.80E-01} & \num{1.40E-01} & \num{3.39E-01} \\
\cmidrule{2-13} 
%
%
\multirow{6}{*}{\textbf{100}} & \textbf{DCGAN} & \textbf{FID} & 811.17 & 653.95 & 868.09 & 652.92 & 801.89 & 508.13 & 831.68 & 751.98 & 598.32 & 662.39 \\
 &  & \textbf{SSIM} & \num{2.69E-01} & \num{5.14E-01} & \num{2.21E-01} & \num{2.89E-01} & \num{2.74E-01} & \num{1.87E-01} & \num{1.91E-01} & \num{4.03E-01} & \num{1.01E-01} & \num{3.22E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 316.33 & 308.52 & 415.98 & 342.83 & 356.37 & 422.05 & 360.53 & 549.11 & 458.04 & 536.61 \\
 &  & \textbf{SSIM} & \num{2.70E-01} & \num{4.97E-01} & \num{2.11E-01} & \num{2.80E-01} & \num{2.33E-01} & \num{1.45E-01} & \num{1.56E-01} & \num{3.86E-01} & \num{1.47E-01} & \num{3.32E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{236.04} & \textbf{217.90} & \textbf{258.82} & \textbf{262.66} & \textbf{218.49} & \textbf{305.15} & \textbf{276.50} & \textbf{400.36} & \textbf{304.54} & \textbf{333.63} \\
 &  & \textbf{SSIM} & \num{2.94E-01} & \num{5.09E-01} & \num{2.04E-01} & \num{3.00E-01} & \num{2.38E-01} & \num{1.62E-01} & \num{1.59E-01} & \num{3.86E-01} & \num{1.41E-01} & \num{3.34E-01} \\

\bottomrule
\end{tabular}%
}
\caption{Detailed FID and SSIM on Fashion-MNIST}
\label{tb_fashion}
\end{table}

==> tables/tb_milestone.tex <==
% \setlength{\tabcolsep}{18pt}
\begin{longtable}{|p{1.7cm}|p{7cm}|p{2cm}|p{2cm}|}
\caption{Project Milestones and Schedule}
\label{milestone}\\


\hline
\rowcolor[HTML]{FFCE93} 
\textbf{Milestone} & \textbf{Tasks} & \textbf{Reporting} & \textbf{End Date} \\ \hline
Week-1 & \begin{tabular}[c]{@{}l@{}}Literature Review: \\Traditional approaches for handling class\\imbalance (i.e. data-centric, model-centric\\and hybird method)
\end{tabular} &
\begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 15-08-2021 \\ \hline

Week-2 & \begin{tabular}[c]{@{}l@{}}Literature Review: \\Generative models and their applications\\for handling class imbalance\\ (i.e. GAN-based and VAE-based)\\Methodologies Exploration: \\Propose different frameworks and discuss\\within the team
\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 22-08-2021 \\ \hline

Week-3 & \begin{tabular}[c]{@{}l@{}}Literature Review: Medical imaging\\domain on class imbalance\\Research Domain Set Up
\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 29-08-2021 \\ \hline

Week-4 & \begin{tabular}[c]{@{}l@{}}GAN exploration on components and\\training strategies\\Datasets Exploration with statistical\\analysis
\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 05-09-2021 \\ \hline

\rowcolor[HTML]{FFCCC9} Week-5 & Proposal Report Finalization & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 12-09-2021 \\ \hline

Week-6 & \begin{tabular}[c]{@{}l@{}}BAGAN-GP experiments on MNIST, \\Fashion-MNIST and CIFAR10. Binary \\classification setting with imbalance \\rates of 1, 5, 10, 20, 50 and 100.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 19-09-2021 \\ \hline
Week-7 & \begin{tabular}[c]{@{}l@{}}BAGAN-GP experiments on Medical\\Imaging Data: Cells and BreakHis. \\Architecture exploration and adjustment \\based on BAGAN-GP\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 26-09-2021 \\ \hline
Week-8 & \begin{tabular}[c]{@{}l@{}}Develop our proposed model CAP-GAN: \\the CVAE component, new objective \\function and new GAN framework\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 10-10-2021 \\ \hline
\rowcolor[HTML]{FFCCC9} Week-9 & \begin{tabular}[c]{@{}l@{}} Complete the progress report. \\Implement pre-training for CVAE. \\BAGAN-GP experiments on MNIST, \\Fashion-MNIST and CIFAR10. 10-class \\classification setting with imbalance \\rates of 1, 5, 10, 20, 50 and 100.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 17-10-2021 \\ \hline

Week-10 & \begin{tabular}[c]{@{}l@{}}
Adjust the architecture of the proposed \\method. Conduct hyperparameter tuning \\for the proposed model. Evaluate the \\proposed model on all benchmark \\datasets. Re-evaluated BAGAN-GP for \\samples of different dimensions.
\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 24-10-2021 \\ \hline
Week-11 &\begin{tabular}[c]{@{}l@{}} Optimize the model performance in terms \\of the inference speed. Re-evaluate the \\optimized model. Summerize results and \\findings. Finalize the project title and \\model name. Draft the final report and \\finalize the documentations.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 31-10-2021 \\ \hline
 Week-12 &  \begin{tabular}[c]{@{}l@{}}
Develop the additional baseline model \\(i.e. conditional DCGAN). Evaluate \\the performance of the additional \\baseline model.
\\ Final report writing.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 07-11-2021 \\ \hline
\rowcolor[HTML]{FFCCC9} Week-13 &\begin{tabular}[c]{@{}l@{}} Finalize all results and documentations. \\Finalize the final report, presentation and \\artefacts. \end{tabular}& \begin{tabular}[c]{@{}l@{}}Ali Braytee\\ Ali Anaissi\end{tabular} & 14-11-2021 \\ \hline



\end{longtable}

==> tables/tb_mnist.tex <==
% \begin{sidewaystable}[!htbp]
\begin{table}[!htbp]
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{rlcrrrrrrrrrr}
\toprule
 & \multicolumn{1}{l}{} &  & \multicolumn{10}{c}{\textbf{Classes}} \\
 \begin{tabular}[c]{@{}r@{}}Imbalance\\ Rate\end{tabular} & Model &  & \textbf{0 (majority)} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} \\
\midrule
%
%
\multirow{6}{*}{\textbf{5}} & \textbf{DCGAN} & \textbf{FID} & 207.93 & 231.91 & 574.02 & 212.52 & 270.49 & 201.67 & 210.00 & 203.94 & 189.60 & 167.79 \\
 &  & \textbf{SSIM} & \num{2.96E-01} & \num{4.67E-01} & \num{1.75E-01} & \num{2.38E-01} & \num{2.28E-01} & \num{1.67E-01} & \num{2.29E-01} & \num{2.91E-01} & \num{2.30E-01} & \num{2.91E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 157.39 & \textbf{240.85} & 150.71 & 170.86 & 252.38 & 161.60 & 128.34 & 169.61 & 145.99 & 165.04 \\
 &  & \textbf{SSIM} & \num{2.86E-01} & \num{4.64E-01} & \num{1.71E-01} & \num{2.35E-01} & \num{2.20E-01} & \num{1.71E-01} & \num{2.36E-01} & \num{2.94E-01} & \num{2.16E-01} & \num{2.97E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{157.16} & 242.23 & \textbf{147.62} & \textbf{165.08} & \textbf{206.09 }& \textbf{154.53} & \textbf{127.52} & \textbf{145.89} & \textbf{145.70} & \textbf{155.65} \\
 &  & \textbf{SSIM} & \num{2.79E-01} & \num{4.74E-01} & \num{1.91E-01} & \num{2.49E-01} & \num{2.28E-01} & \num{1.80E-01} & \num{2.49E-01} & \num{3.09E-01} & \num{2.32E-01} & \num{3.08E-01} \\
\cmidrule{2-13}
%
%

\multirow{6}{*}{\textbf{10}} & \textbf{DCGAN} & \textbf{FID} & 528.09 & 242.10 & 180.30 & 206.94 & 250.58 & 230.72 & 201.96 & 228.18 & 187.70 & 192.01 \\
 &  & \textbf{SSIM} & \num{3.36E-01} & \num{4.58E-01} & \num{1.87E-01} & \num{2.27E-01} & \num{2.38E-01} & \num{1.70E-01} & \num{2.49E-01} & \num{2.68E-01} & \num{2.27E-01} & \num{2.97E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 165.08 & 282.54 & 155.78 & 178.82 & 237.48 & 177.91 & \textbf{138.46} & 198.25 & 159.68 & 158.06 \\
 &  & \textbf{SSIM} &  \num{2.70E-01} & \num{4.66E-01} & \num{1.74E-01} & \num{2.34E-01} & \num{2.32E-01} & \num{1.72E-01} & \num{2.44E-01} & \num{3.10E-01} & \num{2.29E-01} & \num{2.98E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{160.12} & \textbf{250.68} & \textbf{145.18} & \textbf{174.58} & \textbf{225.67} & \textbf{177.76} & 146.50 & \textbf{163.00} & \textbf{157.12} & \textbf{154.49} \\
 &  & \textbf{SSIM} & \num{2.90E-01} & \num{4.78E-01} & \num{1.79E-01} & \num{2.40E-01} & \num{2.28E-01} & \num{1.72E-01} & \num{2.48E-01} & \num{2.98E-01} & \num{2.30E-01} & \num{3.01E-01} \\
\cmidrule{2-13}
%
%

\multirow{6}{*}{\textbf{20}} & \textbf{DCGAN} & \textbf{FID} & 210.22 & 344.15 & 508.33 & 184.82 & 317.27 & 205.03 & 184.93 & 301.06 & 239.51 & 224.13 \\
 &  & \textbf{SSIM} & \num{2.85E-01} & \num{4.69E-01} & \num{2.06E-01} & \num{2.06E-01} & \num{2.31E-01} & \num{1.65E-01} & \num{2.70E-01} & \num{3.23E-01} & \num{2.43E-01} & \num{3.02E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 174.21 & 257.86 & 178.63 & 180.72 & 244.97 & \textbf{186.60} & 138.85 & 210.84 & 171.13 & 171.02 \\
 &  & \textbf{SSIM} &  \num{2.78E-01} & \num{4.68E-01} & \num{1.75E-01} & \num{2.28E-01} & \num{2.40E-01} & \num{1.74E-01} & \num{2.49E-01} & \num{3.19E-01} & \num{2.24E-01} & \num{3.22E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{149.04} & \textbf{219.41} & \textbf{161.04} & \textbf{155.32} & \textbf{243.29} & 188.62 & \textbf{136.91} & \textbf{147.25} & \textbf{156.50} & \textbf{154.00} \\
 &  & \textbf{SSIM} & \num{2.86E-01} & \num{4.63E-01} & \num{1.88E-01} & \num{2.47E-01} & \num{2.31E-01} & \num{1.87E-01} & \num{2.59E-01} & \num{3.03E-01} & \num{2.38E-01} & \num{3.12E-01} \\
\cmidrule{2-13}
%
%

\multirow{6}{*}{\textbf{50}} & \textbf{DCGAN} & \textbf{FID} & 722.07 & 528.49 & 619.79 & 350.49 & 483.00 & 435.90 & 558.23 & 419.34 & 519.03 & 402.41 \\
 &  & \textbf{SSIM} & \num{3.13E-01} & \num{3.58E-01} & \num{1.68E-01} & \num{2.13E-01} & \num{2.43E-01} & \num{2.32E-01} & \num{2.36E-01} & \num{3.10E-01} & \num{2.08E-01} & \num{3.26E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & \textbf{149.28} & 250.79 & 197.96 & 180.09 & 277.71 & 200.27 & 163.66 & 176.13 & 194.40 & 201.32 \\
 &  & \textbf{SSIM} &  \num{2.79E-01} & \num{4.58E-01} & \num{1.77E-01} & \num{2.30E-01} & \num{2.23E-01} & \num{1.66E-01} & \num{2.47E-01} & \num{2.99E-01} & \num{2.27E-01} & \num{2.91E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & 163.90 & \textbf{233.15} & \textbf{157.93} & \textbf{156.78} & \textbf{242.64} & \textbf{173.47} & \textbf{145.42} & \textbf{160.22} & \textbf{148.28} & \textbf{170.29} \\
 &  & \textbf{SSIM} & \num{2.83E-01} & \num{4.69E-01} & \num{1.72E-01} & \num{2.33E-01} & \num{2.14E-01} & \num{1.66E-01} & \num{2.50E-01} & \num{2.90E-01} & \num{2.30E-01} & \num{3.04E-01} \\
\cmidrule{2-13}
%
%

\multirow{6}{*}{\textbf{100}} & \textbf{DCGAN} & \textbf{FID} & 711.49 & 505.38 & 418.74 & 565.95 & 449.87 & 605.25 & 456.66 & 494.41 & 544.54 & 561.03 \\
 &  & \textbf{SSIM} & \num{1.68E-01} & \num{1.50E-01} & \num{1.13E-01} & \num{1.40E-01} & \num{2.78E-01} & \num{8.79E-02} & \num{2.43E-01} & \num{1.83E-01} & \num{1.63E-01} & \num{2.91E-01} \\
 & \textbf{BAGAN-GP} & \textbf{FID} & 167.74 & 237.99 & 215.68 & 203.27 & 280.70 & 230.98 & 228.46 & 228.21 & 221.93 & 206.48 \\
 &  & \textbf{SSIM} &  \num{2.79E-01} & \num{4.62E-01} & \num{1.77E-01} & \num{2.09E-01} & \num{2.30E-01} & \num{1.55E-01} & \num{2.47E-01} & \num{2.85E-01} & \num{2.27E-01} & \num{2.92E-01} \\
 & \textbf{CAP-GAN} & \textbf{FID} & \textbf{160.88} & \textbf{210.50} & \textbf{154.40} & \textbf{155.25} & \textbf{202.50} & \textbf{173.52} & \textbf{139.23} & \textbf{166.63} & \textbf{153.39} & \textbf{156.62 }\\
 &  & \textbf{SSIM} & \num{2.81E-01} & \num{4.83E-01} & \num{1.69E-01} & \num{2.33E-01} & \num{2.35E-01} & \num{1.70E-01} & \num{2.71E-01} & \num{2.91E-01} & \num{2.25E-01} & \num{3.12E-01} \\
%
%

\bottomrule
\end{tabular}%
}
\caption{Detailed FID and SSIM on MNIST}
\label{tb_mnist}
\end{table}

==> tables/tb_time.tex <==

\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrr}
\toprule
Dataset      & Each CVAE Epoch (s)  & Each GAN Epoch (s) \\ \cmidrule{1-3} 
MNIST         & 3.34 & 55.45                  \\
Fashion-MNIST & 3.43 & 55.80                  \\
CIFAR10       & 3.94 & 90.44                 \\
Cells         & 2.06 & 41.13            \\
BreakHis      & 0.79 & 32.70                \\ 
\bottomrule
\end{tabular}%
}
\caption{Estimation of Computational Time for Different Datasets}
\label{tb_time}
\end{table}
